Semi-parametric efficient estimation of small genetic effects in large-scale population cohorts

Population genetics seeks to quantify DNA variant associations with traits or diseases, as well as interactions among variants and with environmental factors. Computing millions of estimates in large cohorts in which small effect sizes are expected, necessitates minimising model-misspecification bias to control false discoveries. We present TarGene, a unified statistical workflow for the semi-parametric efficient and double robust estimation of genetic effects including k-point interactions among categorical variables in the presence of confounding and weak population dependence. k-point interactions, or Average Interaction Effects (AIEs), are a direct generalisation of the usual average treatment effect (ATE). We estimate AIEs with cross-validated and/or weighted versions of Targeted Minimum Loss-based Estimators (TMLE) and One-Step Estimators (OSE). The effect of dependence among data units on variance estimates is corrected by using sieve plateau variance estimators based on genetic relatedness across the units. We present extensive realistic simulations to demonstrate power, coverage, and control of type I error. Our motivating application is the targeted estimation of genetic effects on trait, including two-point and higher-order gene-gene and gene-environment interactions, in large-scale genomic databases such as UK Biobank and All of Us. All cross-validated and/or weighted TMLE and OSE for the AIE k-point interaction, as well as ATEs, conditional ATEs and functions thereof, are implemented in the general purpose Julia package TMLE.jl. For high-throughput applications in population genomics, we provide the open-source Nextflow pipeline and software TarGene which integrates seamlessly with modern high-performance and cloud computing platforms.

==> tabs/MFI_vs_cor_numerics.tex <==


\begin{figure}[ht]

%\hspace{-1.0cm}
\begin{minipage}[]{0.2\textwidth}
	\scalebox{0.8}{\input{tikz/chain}}
\end{minipage}
\begin{minipage}[t]{0.7\textwidth}
\scalebox{0.8}{
\footnotesize{
	\begin{tabular}{lrrrrrrr}
		\toprule
        \multicolumn{8}{l}{Chain}\\
        \toprule
		      Genes &  Interaction &      F &  $\rho_p$ &  p-val &  Partial $\rho_p$ &  p-val &     MI \\
		\midrule
		     $[0, 1]$ &        4.281 &  0.000 &         0.790 &             0.0 &         0.635 &       0.000e+00 &  0.515 \\
		     $[0, 2]$ &        0.056 &  0.117 &         0.622 &             0.0 &         0.031 &       2.261e-23 &  0.301 \\
		     $[1, 2]$ &        4.249 &  0.000 &         0.786 &             0.0 &         0.628 &       0.000e+00 &  0.510 \\
		  $[0, 1, 2]$ &       -0.052 &  0.217 &           NaN &             NaN &           NaN &             NaN &  0.300 \\
		\bottomrule
		\end{tabular}}}
	% \caption{Chain \label{tab:firstDAG}}
	\end{minipage}



\vspace{0.5cm}
\begin{minipage}[]{0.2\textwidth}
	\scalebox{0.8}{\input{tikz/fork}}
\end{minipage}
\begin{minipage}[t]{0.7\textwidth}
\scalebox{0.8}{
\footnotesize{
	\begin{tabular}{lrrrrrrr}
		\toprule
        \multicolumn{8}{l}{Fork}\\
        \toprule
		      Genes &  Interaction &      F &  $\rho_p$ &  p-val &  Partial $\rho_p$ &  p-val &     MI \\
		\midrule
		     $[0, 1]$ &        4.268 &  0.000 &         0.789 &             0.0 &         0.634 &       0.000e+00 &  0.514 \\
		     $[0, 2]$ &        4.257 &  0.000 &         0.788 &             0.0 &         0.632 &       0.000e+00 &  0.512 \\
		     $[1, 2]$ &       -0.014 &  0.376 &         0.622 &             0.0 &         0.028 &       6.518e-19 &  0.300 \\
		  $[0, 1, 2]$ &        0.020 &  0.376 &           NaN &             NaN &           NaN &             NaN &  0.300 \\
		\bottomrule
		\end{tabular}}}
	% \caption{Fork}
	\end{minipage}



\vspace{0.5cm}
\begin{minipage}[]{0.2\textwidth}
	\scalebox{0.8}{\input{tikz/collider}}
\end{minipage}
\begin{minipage}[t]{0.7\textwidth}
\scalebox{0.8}{
\footnotesize{
	\begin{tabular}{lrrrrrrr}
		\toprule
        \multicolumn{8}{l}{Additive collider}\\
        \toprule
		      Genes &  Interaction &      F &  $\rho_p$ &  p-val &  Partial $\rho_p$ &  p-val &     MI \\
		\midrule
		     $[0, 1]$ &        2.144 &  0.000 &         0.395 &           0.000 &         0.505 &       0.000e+00 &  1.154e-01 \\
		     $[0, 2]$ &       -0.989 &  0.000 &        -0.002 &           0.593 &        -0.070 &      5.172e-109 &  2.059e-06 \\
		     $[1, 2]$ &        2.144 &  0.000 &         0.395 &           0.000 &         0.505 &       0.000e+00 &  1.154e-01 \\
		  $[0, 1, 2]$ &        0.003 &  0.438 &           NaN &             NaN &           NaN &             NaN & -2.678e-02 \\
		\bottomrule
		\end{tabular}}}
	% \caption{Additive collider}
	\end{minipage}



\vspace{0.5cm}
\begin{minipage}[]{0.2\textwidth}
	\scalebox{0.8}{\input{tikz/collider}}
\end{minipage}
\begin{minipage}[t]{0.7\textwidth}
\scalebox{0.8}{
\footnotesize{
	\begin{tabular}{lrrrrrrr}
		\toprule
        \multicolumn{8}{l}{Multiplicative collider}\\
        \toprule
		      Genes &  Interaction &      F &  $\rho_p$ &  p-val &  Partial $\rho_p$ &  p-val &     MI \\
		\midrule
		     $[0, 1]$ &        0.032 &  0.140 &         0.427 &           0.000 &         0.478 &       0.000e+00 &  1.403e-01 \\
		     $[0, 2]$ &       -2.156 &  0.000 &        -0.005 &           0.145 &        -0.087 &      1.463e-166 &  1.529e-05 \\
		     $[1, 2]$ &        0.036 &  0.109 &         0.429 &           0.000 &         0.480 &       0.000e+00 &  1.415e-01 \\
		  $[0, 1, 2]$ &        4.237 &  0.000 &           NaN &             NaN &           NaN &             NaN & -1.150e-01 \\
		\bottomrule
		\end{tabular}}}
	% \caption{Multiplicative collider}
	\end{minipage}





\vspace{0.5cm}
\begin{minipage}[]{0.2\textwidth}
	\scalebox{0.8}{\input{tikz/collider_chain}}
\end{minipage}
\begin{minipage}[t]{0.7\textwidth}
\scalebox{0.8}{
\footnotesize{
	\begin{tabular}{lrrrrrrr}
		\toprule
        \multicolumn{8}{l}{Additive collider + chain}\\
        \toprule
		      Genes &  Interaction &      F &  $\rho_p$ &  p-val &  Partial $\rho_p$ &  p-val &     MI \\
		\midrule
		     $[0, 1]$ &        2.103 &  0.000 &         0.705 &             0.0 &         0.362 &             0.0 &  0.396 \\
		     $[0, 2]$ &        3.288 &  0.000 &         0.790 &             0.0 &         0.599 &             0.0 &  0.515 \\
		     $[1, 2]$ &        2.113 &  0.000 &         0.706 &             0.0 &         0.364 &             0.0 &  0.397 \\
		  $[0, 1, 2]$ &        0.050 &  0.162 &           NaN &             NaN &           NaN &             NaN &  0.335 \\
		\bottomrule
		\end{tabular}}}
	% \caption{Additive collider + chain}
	\end{minipage}




\vspace{0.5cm}
\begin{minipage}[]{0.2\textwidth}
	\scalebox{0.8}{\input{tikz/collider_chain}}
\end{minipage}
\begin{minipage}[t]{0.7\textwidth}
\scalebox{0.8}{
\footnotesize{
	\begin{tabular}{lrrrrrrr}
		\toprule
        \multicolumn{8}{l}{Multiplicative collider + chain}\\
        \toprule
		      Genes &  Interaction &      F &  $\rho_p$ &  p-val &  Partial $\rho_p$ &  p-val &     MI \\
		\midrule
		     $[0, 1]$ &       -0.017 &  0.342 &         0.709 &             0.0 &         0.365 &             0.0 &  0.403 \\
	         $[0, 2]$ &        2.094 &  0.000 &         0.786 &             0.0 &         0.596 &             0.0 &  0.510 \\
		     $[1, 2]$ &       -0.057 &  0.092 &         0.707 &             0.0 &         0.361 &             0.0 &  0.401 \\
		  $[0, 1, 2]$ &        4.359 &  0.000 &           NaN &             NaN &           NaN &             NaN &  0.293 \\
		\bottomrule
		\end{tabular}}}
	% \caption{Multiplicative collider + chain\label{tab:lastDAG}}
	\end{minipage}
\caption{\textbf{Here listed are the precise values that led to Fig.~\ref{fig:MFI_vs_correlation_MI}}. From each graph, we generated 100k samples from a Bernoulli distribution with $p=0.5$ and added zero-mean Gaussian noise ($\sigma=0.4$) before binarising. To quantify the significance value of the interactions, we generated 1,000 bootstrap resamples of the data, and calculated $F$: the fraction of resampled interactions that have a different sign from the original interaction. A smaller $F$ corresponds to a more significant interaction. \label{tab:MFI_vs_cor_numerics}}
\end{figure}

